MAEEG: Masked Auto-encoder for EEG Representation Learning

Decoding information from bio-signals such as EEG, using machine learning has been a challenge due to the small data-sets and difficulty to obtain labels. We propose a reconstruction-based self-supervised learning model, the masked auto-encoder for EEG (MAEEG), for learning EEG representations by learning to reconstruct the masked EEG features using a transformer architecture. We found that MAEEG can learn representations that significantly improve sleep stage classification (~5% accuracy increase) when only a small number of labels are given. We also found that input sample lengths and different ways of masking during reconstruction-based SSL pretraining have a huge effect on downstream model performance. Specifically, learning to reconstruct a larger proportion and more concentrated masked signal results in better performance on sleep classification. Our findings provide insight into how reconstruction-based SSL could help representation learning for EEG.

==> sections/abstract.tex <==
  Decoding information from bio-signal data such as EEG using machine learning has been a challenge due to the small data-sets and difficulty to obtain labels. We proposed a reconstruction-based SSL model for learning EEG representations, the masked autoencoder for EEG (MAEEG), inspired by the SSL models proposed in computer vision and speech. MAEEG learns representations for EEG by learning to reconstruct the masked EEG features to the original EEG signals using a transformer architecture. We found that MAEEG can learn representations that significantly improve the sleep stage classification when only a small number of labels was given. We also found that sample length and different ways of masking during MAE pretraining have huge effect on downstream model performance, and that learning to reconstruct a larger proportion and more concentrated masked signal during MAE pretraining results in better performance on sleep classification. 

==> sections/introduction.tex <==
\section{Introduction}
Decoding information from Electroencephalography (EEG) and other biosignal modalities have enabled health-related clinical applications such as sleep pattern detection \citep{ghassemi2018you}. Recently, machine learning models have been effectively applied on classifying EEG signals, mostly via supervised learning \citep{lawhern2018eegnet}. However, such methods rely on a large amount of labels for biosignal data, which are usually difficult and expensive to obtain. One way to improve accuracy when decoding EEG signals using only a small amount of labels is to learn useful representations from unlabeled data via self-supervised learning (SSL). 

SSL has recently been explored in the field of computer vision and speech processing. The idea of SSL is to boost the performance of the main task (i.e.,\ the downstream task) by learning meaningful representations through an SSL task. One way to learn representations is through masking and reconstructing the input signals. For example, \citet{he2022masked} proposed masked auto-encoder (MAE) as an SSL model for computer vision: By masking random patches of the input image and reconstructing the missing pixels using a vision transformer architecture, MAE learns meaningful representations which help achieve high accuracy for the downstream image classification task. Such reconstruction-based SSL methods were also widely used for speech processing: The representations learned from the Wav2Vec series of SSL models significantly improve the performance of various downstream tasks such as automatic speech recognition and speech emotion recognition \citep{baevski2020wav2vec}. Given the success of reconstruction-based SSL methods in other domains, it is desirable to learn whether and how such methods could be adapted to physiological time-series data such as EEG.

In this study, we explore representations learning using reconstruction-based SSL on EEG data. We proposed a new SSL model, MAEEG, which can learn EEG representations by reconstructing the raw signal from masked tokens. We found that MAEEG could learn meaningful representations which yield better performance compared to another reconstruction-based SSL model and a baseline supervised model when the encoder is frozen. We further explore how masking may affect SSL and downstream task performance, and found that in general, a higher probability and more concentrated masking yields better task performance.

==> sections/method.tex <==
\section{Method}



%\subsection{Sleep EEG dataset}
%To examine how reconstruction-based SSL may help learn useful representations for classifying sleep stages from EEG signals, we use the sleep data-set provided from 2018 PhysioNet Challenge \citep{ghassemi2018you}. The dataset contains overnight polysomnography of 994 subjects (i.e.,\ around 7,000 hours of data). The subjects are split into a training set (596 subjects), validation set (198 subjects) and testing set (200 subjects). Each polysomnogram contains simultaneous recordings of EEG, ECG and respiratory signals during sleep and two sets of labels: 5 sleep stages and respiratory-effort related arousals. Here, we focused on using the 6-channel EEG signals to classify 5 stages of sleeping (i.e.,\ wake, N1, N2, N3, REM). 

%\subsection{Model}

\subsection{Reconstruction-based SSL}

In general, SSL is a machine learning method which aims to learn informative representations that could help boost the performance of the main task. Specifically, reconstruction-based SSL is to learn representations by reconstructing the masked, invisible part of the input signals by using the visible contextual information. Our MAEEG model is a reconstruction-based SSL model for learning EEG representations. MAEEG is built based on the architecture of BENDR, an SSL model for EEG proposed by \citet{kostas2021bendr}.

\paragraph{BENDR.} The model architecture of BENDR is illustrated in Figure \ref{fig:SSL_models} A. First, the 6-channel 100Hz raw EEG signals are the input to the 6 convolutional layers which encode the raw EEG into 64-dimensional convolved features ($\sim$1.05Hz). Dropout and GroupNorm were implemented in each convolutional layer and GELU was used as the output activation function. A mask is then generated and applied on the convolved features to ``mask out" the indices specified (i.e., set the activation to specified value $M$) . More concretely, given a sequences $t_i$ with $N$ features $t_1, t_2, t_3...t_N$, and a mask $I_m$ containing indices $i \in I_m$, the features after masking $q_i$ are generated such that:
\begin{equation}
    q_i=
    \begin{cases}
      M \sim \mathcal{N}(0,\,\sqrt{1/64}), & \text{if} \ i \in I_m  \\
      t_i, & \text{otherwise}
    \end{cases}
  \end{equation}
  
The masked tokens are the input to the 8 transformer encoder layers, which encode the convolved features into 192-dimensional output features. The positions are encoded using a convolutional layer which acts as relative positional embedding. The output features are the input to a final convolutional layer to map the features back to 64-dimensional contextual features. The model implements contrastive learning by using contrastive loss (see supplementary) as the SSL loss to learn EEG representations. 

\paragraph{MAEEG.} The MAEEG model has a similar architecture to BENDR, with 6-layer convolutional encoder to encode raw EEG to convolved features. The features are then masked and sent to 8 transformer encoder layers. Different from BENDR which maps the 192 dimensional features to 64 dimensions for contrastive learning, the MAE has two additional layers to map the output transformer features back to the raw EEG dimensions. Reconstruction loss is calculated by comparing the reconstructed EEG ($\hat{x}$) and input EEG ($x$) signals as $1-cosine \ similarity(\hat{x}, x)$ (Figure \ref{fig:SSL_models} B). In summary, the main difference between MAEEG and BENDR is the reconstruction loss for optimizing the encoders: BENDR aims to reconstruct signals in the features space, while MAE tends to reconstruct signals in the raw EEG space. 

\begin{figure*}[ht]
% \vskip 0.2in
% \begin{center}
\centerline{\includegraphics[width=\columnwidth]{figures/Figure1.png}}
\caption{\textbf{SSL model architecture} We compare two reconstruction-based SSL model architecture. \textbf{A.} BENDR learns representations through contrastive loss between convolved and contextual features, while \textbf{B.} MAEEG learns representations through reconstruction loss between input and output EEG signals. }
\label{fig:SSL_models}
% \end{center}
\end{figure*}


\subsection{Features for Downstream classification}
As mentioned, two features are learned by the SSL models - the convolved features, $t_i$, which are the output of the convolutional encoder, and the contextual features, $c_i$, which are the output of the transformer encoder. To build downstream classification model for classifying sleep stages, we preserve most of the SSL architecture with the pretrained encoders, and simply add a fully-connected classification layer which takes the SSL features as input and generates probabilities for predicting the 5 sleep stages (Figure \ref{fig:DS_models}). To better understand representations learned from different stages of training (i.e.,\ SSL pretraining with no labels and downstream supervised training with labels), we conducted two types of downstream classification analyses: (1) To examine low-level features $t_i$ learned solely from the SSL pre-training, we use $t_i$ while ``freezing" the convolutional encoder (meaning that the weights of the encoder are fixed) during downstream classification. Only the classification layer gets trained in this condition (Figure \ref{fig:DS_models} A); (2) To examine the pre-trained model as an initialization for supervised training, we use $c_i$ while fine-tuning both convolutional and transformer encoders and the classification layer during downstream classification (Figure \ref{fig:DS_models} B). For (2), to determine which transformer layer contains the most useful SSL features for classification, we first probed the features from each layer and found that layer 2 showed the best classification performance out of all layers. We therefore extracted $c_i$ from layer 2 as the SSL features to conduct all following analyses. We conducted these analyses on MAEEG, BENDR and a baseline supervised model which has the same architecture as other models but the encoders are randomly initialized, i.e., \ no SSL pretraining prior to the downstream classification task. We applied analyses with various number of subjects or percent of sessions to examine model performance given different amount of labels.

\begin{figure*}[ht]
% \vskip 0.2in
% \begin{center}
\centerline{\includegraphics[width=\columnwidth]{figures/Figure1_1.png}}
\caption{\textbf{Downstream model architecture} \textbf{A.} Classification using convolved features $t_i$ with encoder frozen to examine the representation learned solely by SSL without labels.  \textbf{B.} Classification using contextual features $c_i$. The encoders are fine-tuned during downstream training to examine the pre-trained model as an initialization for supervised training.}
\label{fig:DS_models}
% \end{center}
\end{figure*}



\subsection{Masking effect analyses}
The masking during SSL pretraining determines the difficulty of the SSL task, and the representations learned from such task. Therefore, it is critical to understand what could be an ideal way of masking for learning EEG signals. In the original BENDR, they set a probability (p=0.065) for each token to be the beginning of a mask with a length of 10 tokens. The problem with this is that for each sequence, the mask can vary a lot - sometimes most of the tokens can be masked with overlap, and sometimes there is no token being masked - which may cause the instability of representation learning. Here, we tried to use a more systematic way to generate the mask, by determining the mask rate and the number of mask chunks. These two factors would determine how long each mask looks like, as illustrated in Figure\ref{fig:mask_result}A. We did two analyses: 
\begin{enumerate}
    \item  Pretrained the models with 3 mask rates: 75\%, 50\% and 25\%, and 3 numbers of mask chunks: 1, 5, and 10.
    \item Pretrained models with single mask chunk but vary the mask span to further confirm the effects.
\end{enumerate}
The resulting pretrained models were evaluated by the downstream performance when using the learned features for classification.
% (1) We pretrained the models with 3 mask rates : 75\%, 50\% and 25\%, and 3 numbers of mask chunks: 1, 5, and 10. (2) Based on the results from (1) that models with single mask chunk and higher mask rate seems to perform better, we pretrained models with single mask chunk but vary the mask span to further confirm the effects. 
We conducted all the analyses on BENDR and MAEEG pretrained on 100s samples because models pretrained on 30s samples did not have enough tokens for examining the effect of these mask variations. 
\label{sec:mask_effect}



==> sections/related.tex <==
\section{Background and Related Work}
While SSL methods have been widely applied in domains such as computer vision, natural language processing and speech processing, it remains unclear how SSL could be used on bio-signal data such as EEG to learn useful representations. A typical SSL for learning time-series data is to learn the temporal relationships between time-series samples. For example,  \cite{banville2021uncovering} applied: relative positioning, temporal shuffling and contrastive predictive coding, and showed that SSL-pretrained encoder could produce features that outperformed supervised learning when there is only a small amount of labeled data. The three proposed SSL tasks share some similarities that all of them encourage the encoder to learn features that discriminate samples that are close or distant in time. This would be helpful for classification tasks under the assumption that samples closer in time tend to have the same labels compared to samples further away. 

Another category of SSL for time-series data is the reconstruction-based SSL. A series of reconstruction-based SSL models was first proposed for speech processing \citep{baevski2020wav2vec}. In reconstruction-based SSL, after the raw time-series input was encoded in the feature space, part of the features get ``masked" (i.e.\ the features were set to 0) before sending to the transformer layers. The SSL task is to use transformer model to reconstruct the masked part of the features by using the remaining contextual features. The learning is optimized by using contrastive learning, i.e.\ the loss is calculated by contrasting the similarity between the reconstructed features and the true unmasked features vs. the negative counterparts. Inspired by the Wav2vec2 model, \citet{kostas2021bendr} proposed BENDR, a reconstruction-based SSL for processing EEG signals. In \citet{kostas2021bendr}, BENDR was proposed to use massive data (i.e.,\ the TUH dataset) to learn EEG representations and aim to adapt the pretrained model to various downstream EEG tasks with various data-sets collected independently from the pretraining data-set. While the results showed that BENDR pretraining seems to improve several downstream tasks compared to random initialized models, the results are not consistent across different data-sets/tasks. Furthermore, when the encoder was frozen, the classification accuracy dropped to only marginally above chance for 4 out of 5 tasks, suggesting that EEG representations learned from BENDR pretraining could not directly benefit the downstream tasks without fine-tuning. The results could be due to the non-generalizable factors introduced by the different data-sets used during pretraining and downstream stages, such as the different lengths of samples or little transferable EEG features when subjects were performing different tasks. Overall, it remains under-investigated if the reconstruction-based SSL methods could learn useful representations for EEG signals. 

In this study, we aim to examine whether reconstruction-based SSL methods are effective for learning EEG representations, and how different ways of masking would affect representation learning. Specifically, we proposed a new model, masked auto-encoder for learning EEG representations (MAEEG), which is inspired by both BENDR and the masked autoencoders applied in computer vision \citep{he2022masked}, to broaden our understanding of reconstruction-based SSL for EEG. The key difference between BENDR and MAEEG is that instead of learning to reconstruct the features through constrastive learning like BENDR, MAEEG learns to reconstruct the raw EEG signals by minimizing the reconstruction loss. We show that by learning to reconstruct the raw signal, MAEEG is able to learn better representations for discriminating sleep stages than BENDR by pretraining only, and both reconstruction-based methods are effective for learning EEG representations. We also show that different ways of masking have a large effect on representation learning and downstream classification performance, and such effects were found in both BENDR and MAEEG. 










==> sections/results.tex <==
\section{Results}

\subsection{Sleep EEG dataset}
To examine how reconstruction-based SSL may help learn useful representations for classifying sleep stages from EEG signals, we use the sleep data-set provided from 2018 PhysioNet Challenge \citep{ghassemi2018you}. The dataset contains overnight polysomnography of 994 subjects (i.e.,\ around 7,000 hours of data). The subjects are split into a training set (596 subjects), validation set (198 subjects) and testing set (200 subjects). Each polysomnogram contains simultaneous recordings of EEG, ECG and respiratory signals during sleep and two sets of labels: 5 sleep stages and respiratory-effort related arousals. Here, we focused on using the 6-channel EEG signals to classify 5 stages of sleeping (i.e.,\ wake, N1, N2, N3, REM). All the models and experiments presented in this section are built and run on Pytorch 1.8.1.

\subsection{MAEEG learned useful representations for classifying sleep stages}
We first examine convolved features learned solely by SSL pretraining by freezing the convolutional encoders when performing the sleep stage classification task. We found that representations pretrained by MAE (both 30s and 100s samples) significantly outperform the representations trained by BENDR and the supervised baseline model across different amount of subjects for training (Figure \ref{fig:ssl_performance} A). This suggests that representations learned from MAE pretraining did capture features that are useful for classifying sleeping stages.   

We next examine the model performance using contextual features when fine-tuning the encoders during the sleep stage classification task. We found that when only given one subject's labels (containing all sleep stages), MAEEG pretrained on 100s (MAE-100s) outperformed other models, while BENDR pretrained on 30s (BENDR-30s) performed the best on 10 subjects' and 50 subjects' labels. We got the best classification performance (90 \% accuracy) from MAE-100s. Interestingly, we found that MAE-100s performed significantly better compared to MAE-30s, and we found an opposite effect on BENDR - BENDR-30s performed significantly better compared to BENDR-100s, suggesting that representations learned from the two reconstruction-based SSL models are distinct and the sample length for pretraining has a big effect on downstream performance. Also, the advantage of MAEEG-pretrained convolved features did not reflect in model performance when the encoders were fine-tuned, suggesting that though MAE may learn some useful features to discriminate sleep stages through pretraining, such pretraining can also affect the models' ability to learn at the same time. 


\begin{figure*}[ht]
% \vskip 0.2in
% \begin{center}
\centerline{\includegraphics[width=\columnwidth]{figures/Figure2.png}}
\caption{\textbf{Model comparison on classifying sleep stages} \textbf{A.} Classification performance with different numbers of downstream subjects using convolved features when the encoders were frozen. MAE pretrained on 30s and 100s performed significantly better than BENDR models and baseline supervised model. \textbf{B.} Classification performance with different numbers of downstream subjects using contextual features when the encoders were fine-tuned. }
\label{fig:ssl_performance}
% \end{center}
\end{figure*}


\subsection{Masking effects in MAE}
Next, we examined how different ways of masking during reconstruction-based SSL pretraining may affect representation learning and downstream classification performance using contextual feature $c_i$ with finetuning. As mentioned in Section \ref{sec:mask_effect}, we vary the mask rate the number of mask chunks to examine how different style of masking during MAE pretraining would affect downstream performance. We first examined the SSL loss during pretraining, and found that higher percentage of masking with less chunks (which yields longer masks) is the most difficult to train (supplementary figure). We then examined the downstream model performance and found that the model performances differ the most when given the least amount of labels - such as 0.1\% (i.e.\ $\sim$4 hours of labels) of downstream training data (Figure \ref{fig:mask_result}B). With such small amount of labels, we found that masking 75\% of the tokens performed better overall compared to masking 50\% and 25\% of the tokens, and models with single chunk performed better than models with multiple chunks. All models with MAE pretraining performed better than the models without pretraining (Figure \ref{fig:mask_result}C). Finally, we examined whether such trend (single chunk with longer mask performs better) preserved when we vary the mask span of a single mask chunk, and whether it generalizes to BENDR. We found a consistent pattern that when models pretrained with longer mask span performs better than models pretrained with shorter mask span when there only a small amount of labels, and such pattern generalized to BENDR (Figure \ref{fig:mask_result}D). This finding is likely due to the fact that a single and long mask during pretraining forced the model to learn a more difficult task and yield more useful representations for sleep staging classification.  


\begin{figure*}[ht]
% \vskip 0.2in
% \begin{center}
\centerline{\includegraphics[width=\columnwidth]{figures/Figure3.png}}
\caption{\textbf{Masking effect on classification performance} \textbf{A.} Example of generating different masks for SSL pretraining by varying the mask rate and number of mask chunks. \textbf{B.} Classification performance using fine-tuned contextual features with various masking conditions and percentage of training sessions. \textbf{C.} Classification results using 0.1 \% of labels with different masking conditions. Overall, we found that masking 75\% of the signals with 1 chunk results in the best performance. \textbf{D.} Classification results using 0.1 \% of labels when varying the masking span. We found that longer mask span yields better results for both MAE-100s and BENDR-100s. np = no pretrain}
\label{fig:mask_result}
% \end{center}
\end{figure*}

\subsection{Attention learned from SSL}
To understand how the EEG representation learned from reconstruction-based SSL help sleep classification, we visualized the attention from the transformer layer where features were extracted (i.e.\ layer 2) after SSL pretraining but before extensive downstream supervised training (we slightly tuned the models with 1 epoch with 1 subjects' of data just to get stable representations.) We extract the The token-by-token attention maps for the baseline supervised model and the models pretrained by MAE and BENDR. We visualized the attention maps from a sample where the label is N2 (Figure \ref{fig:attention}). Compared to the attention from baseline models which is equally distributed as shown in Figure\ref{fig:attention}A, MAE- and BENDR- pretrained models showed distinct attention patterns learned from pretraining. Interestingly, we observed that MAE-100s and MAE-30s actually learned very different attention patterns, with MAE-30s learning to attend locally to neighboring tokens while MAE-100s learning to attend more distant tokens (Figure\ref{fig:attention}B). On the other hand, BENDR-100s and BENDR-30s also learned very different attention patterns, with BENDR-100s learning to attend locally and BENDR-30s learning a more global distributed attention. This suggests that representation learning can be very different based not only on the model architecture, but also on subtle SSL settings such as the length of pretraining samples. Moreover, MAE-30s and BENDR-100s performed worse on the classification task compared to their counterparts (Figure \ref{fig:ssl_performance}B), suggesting that local attention acquired from pretraining may not be desirable for the sleep staging classification task.


\begin{figure*}[ht]
% \vskip 0.2in
% \begin{center}
\centerline{\includegraphics[width=\columnwidth]{figures/Figure4.png}}
\caption{\textbf{Visualizing attention after pretraining} \textbf{A.} Initialized attention. \textbf{B.} (left) attention learned from MAE-30s pretraining; (right) attention learned from MAE-100s pretraining \textbf{C.} (left) attention learned from BENDR-30s pretraining; (right) attention learned from BENDR-100s pretraining.}
\label{fig:attention}
% \end{center}
\end{figure*}
